Resilience patterns in higher-order meta-population networks

Meta-population networks are effective tools for capturing population movement across distinct regions, but the assumption of well-mixed regions fails to capture the reality of population higher-order interactions. As a multidimensional system capturing mobility characteristics, meta-population networks are inherently complex and difficult to interpret when subjected to resilience analysis based on N-dimensional equations. We propose a higher-order meta-population model that captures large-scale global cross-regional mobility and small-scale higher-order interactions within regions. Remarkably, we extend the dimension-reduction approach, simplifying the N-dimensional higher-order meta-population system into a one-dimensional equation by decomposing different network behaviours into a single universal resilience function, thereby allowing for convenient and accurate prediction of the system resilience. The network structure and human mobility parameters can clearly and simply express the epidemic threshold. Numerical experimental results on both real networks and star networks confirm the accuracy of the proposed dimension-reduction framework in predicting the evolution of epidemic dynamics on higher-order meta-population networks. Additionally, higher-order interactions among populations are shown to lead to explosive growth in the epidemic infection size potentially. Population mobility causes changes in the spatial distribution of infectious diseases across different regions.

==> ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}

% Sets running headers as well as PDF title and authors
\headers{An Example Article}{D. Doe, P. T. Frank, and J. E. Smith}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{Resilience patterns in higher-order meta-population networks
\thanks{Submitted to the editors DATE.
\funding{This work was partially supported by the Social Science Foundation of Chongqing, No. 2021PY53, Natural Science Foundation of Chongqing, No. cstc2021jcyj-msxmX0132, Natural Science Foundation of Yuzhong District, Chongqing, No. 20210117, and National Natural Science Foundation of China under Grants No. 61903266 and No. 62272074.}}}

% Authors: full names plus addresses.
\author{Yanyi Nie\thanks{College of Computer Science, Sichuan University, Chengdu 610065 (\email{nienienie@stu.scu.edu.cn}, \email{lintao@scu.edu.cn}).}
\and Tao Lin\footnotemark[2]
\and Yanbing Liu\thanks{Chongqing Medical University, Chongqing, 400016, China (\email{liuyb@cqupt.edu.cn}).}
\and Wei Wang \thanks{School of Public Health, Chongqing Medical University, Chongqing, 400016, China (\email{wwzqbx@hotmail.com}).}}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 

